Spontaneous spin bifurcations and ferromagnetic phase transitions in a spinor exciton-polariton condensate

We observe a spontaneous parity breaking bifurcation to a ferromagnetic state in a spatially trapped exciton-polariton condensate. At a critical bifurcation density under nonresonant excitation, the whole condensate spontaneously magnetizes and randomly adopts one of two elliptically polarized (up to 95% circularly-polarized) states with opposite handedness of polarization. The magnetized condensate remains stable for many seconds at 5 K, but at higher temperatures it can flip from one magnetic orientation to another. We optically address these states and demonstrate the inversion of the magnetic state by resonantly injecting 100-fold weaker pulses of opposite spin. Theoretically, these phenomena can be well described as spontaneous symmetry breaking of the spin degree of freedom induced by different loss rates of the linear polarizations.

==> mainwhole_aux <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldcontentsline\contentsline
\gdef\contentsline#1#2#3#4{\oldcontentsline{#1}{#2}{#3}}
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\contentsline\oldcontentsline
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax 
\gdef\HyperFirstAtBeginDocument#1{#1}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{deng_condensation_2002,kasprzak_bose-einstein_2006,balili_bose-einstein_2007,baumberg_spontaneous_2008,ohadi_spontaneous_2012}
\citation{nelsen_dissipationless_2013}
\citation{sturm_all-optical_2014,dreismann_coupled_2014}
\citation{amo_exciton-polariton_2010,ballarini_all-optical_2013,cerna_ultrafast_2013}
\citation{nguyen_realization_2013,bhattacharya_solid_2013,schneider_electrically_2013}
\citation{buluta_quantum_2009}
\citation{aleiner_radiative_2012,zhang_weak_2015}
\citation{lagoudakis_stimulated_2002,martin_polarization_2002,kavokin_polarization_2003,kavokin_quantum_2004,renucci_microcavity_2005,krizhanovskii_rotation_2006,gippius_polarization_2007,leyder_observation_2007,paraiso_multistability_2010,gao_polariton_2012,kammann_nonlinear_2012,takemura_polaritonic_2014}
\citation{kavokin_microcavities_2007}
\citation{savvidis_angle-resonant_2000}
\citation{wertz_spontaneous_2010}
\citation{askitopoulos_polariton_2013}
\citation{bloch_ultracold_2005}
\citation{wertz_spontaneous_2010,wouters_excitations_2007,tosi_sculpting_2012}
\newlabel{FirstPage}{{}{1}{}{section*.1}{}}
\@writefile{toc}{\contentsline {title}{Spontaneous spin bifurcations and ferromagnetic phase transitions in a spinor exciton-polariton condensate}{1}{section*.2}}
\@writefile{toc}{\contentsline {abstract}{Abstract}{1}{section*.1}}
\newlabel{sec:intro}{{I}{1}{}{section*.3}{}}
\@writefile{toc}{\contentsline {section}{\numberline {I}Introduction}{1}{section*.3}}
\citation{shelykh_polarization_2006}
\citation{deng_condensation_2002,kasprzak_bose-einstein_2006}
\citation{martin_polarization_2002,shelykh_semiconductor_2004,krizhanovskii_rotation_2006,roumpos_signature_2009,ohadi_spontaneous_2012}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces (a) Scanning electron microscopy image of a membrane microcavity, cleaved across the middle. The membrane allows resonant excitation from the back side of the cavity. (b) Above threshold hot polaritons condense into a single coherent state located at the center of the trap (pump spots shown by dashed circles), which is found at $k_\parallel =0$ (c). The spin state of the condensate is determined by studying the emission polarization.}}{2}{figure.1}}
\newlabel{fig:1}{{1}{2}{(a) Scanning electron microscopy image of a membrane microcavity, cleaved across the middle. The membrane allows resonant excitation from the back side of the cavity. (b) Above threshold hot polaritons condense into a single coherent state located at the center of the trap (pump spots shown by dashed circles), which is found at $k_\parallel =0$ (c). The spin state of the condensate is determined by studying the emission polarization}{figure.1}{}}
\newlabel{sec:circbuildup}{{II}{2}{}{section*.4}{}}
\@writefile{toc}{\contentsline {section}{\numberline {II}Spontaneous buildup of circular polarization}{2}{section*.4}}
\citation{roumpos_signature_2009,ohadi_spontaneous_2012,kammann_nonlinear_2012,li_incoherent_2015}
\citation{deng_condensation_2002,kasprzak_bose-einstein_2006}
\citation{askitopoulos_polariton_2013}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces  (a) Polarization-resolved spatial image of the only two realizations observed in a single trapped condensate in a 4-spot trapping geometry. (b) At $T=\SI {5}{\K }$ the spin-polarized states remain stable for many seconds. (c) Simultaneously measured components of the pseudospin for 1000 realizations. The total degree of polarization is $0.93\pm 0.03$ and the two average pseudospin states are $s_\delimiter "3223379 =[-0.22, 0.19, -0.94]$ (blue vector) and $s_\delimiter "3222378 =[-0.22, -0.14, 0.96]$ (orange vector). The measurement error for each component is $<5\%$, and the variance is $\sim 1\%$.  }}{3}{figure.2}}
\newlabel{fig:Random}{{2}{3}{(a) Polarization-resolved spatial image of the only two realizations observed in a single trapped condensate in a 4-spot trapping geometry. (b) At $T=\SI {5}{\K }$ the spin-polarized states remain stable for many seconds. (c) Simultaneously measured components of the pseudospin for 1000 realizations. The total degree of polarization is $0.93\pm 0.03$ and the two average pseudospin states are $s_\downarrow =[-0.22, 0.19, -0.94]$ (blue vector) and $s_\uparrow =[-0.22, -0.14, 0.96]$ (orange vector). The measurement error for each component is $<5\%$, and the variance is $\sim 1\%$}{figure.2}{}}
\citation{rubo_suppression_2006}
\citation{vladimirova_polariton-polariton_2010,takemura_polaritonic_2014,takemura_heterodyne_2014}
\citation{kasprzak_formation_2008}
\citation{lagoudakis_stimulated_2002}
\citation{paraiso_multistability_2010}
\citation{balili_huge_2010,klopotowski_optical_2006}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces  (a) Emitted circular $\sigma _+$ and $\sigma _-$ intensities for a condensate realization when $P>P_c$, created by a long pulse (marked by P). The condensate randomly picks the $s_\delimiter "3223379 $ state here. Note the opposite axis directions for $\sigma _+$ and $\sigma _-$ components. (b) Same as (a), with pump intensity modulated by square wave (shown on top by P). A cut from the middle of a \SI {9}{\milli \second } exposure is shown, where each square pulse corresponds to a single realization. The condensate randomly picks $s_\delimiter "3222378 $ or $s_\delimiter "3223379 $ states (marked by grey rectangles). (c) Occurrence contrast $\xi $ of spin-up and spin-down realizations measured in (b) vs the ellipticity of the pump. (d) Measured circular polarization of condensate vs pump ellipticity. Dashed lines mark the region where the condensate initializes stochastically in spin-up or spin-down states in each realization.  }}{4}{figure.3}}
\newlabel{fig:pulsetrain}{{3}{4}{(a) Emitted circular $\sigma _+$ and $\sigma _-$ intensities for a condensate realization when $P>P_c$, created by a long pulse (marked by P). The condensate randomly picks the $s_\downarrow $ state here. Note the opposite axis directions for $\sigma _+$ and $\sigma _-$ components. (b) Same as (a), with pump intensity modulated by square wave (shown on top by P). A cut from the middle of a \SI {9}{\milli \second } exposure is shown, where each square pulse corresponds to a single realization. The condensate randomly picks $s_\uparrow $ or $s_\downarrow $ states (marked by grey rectangles). (c) Occurrence contrast $\xi $ of spin-up and spin-down realizations measured in (b) vs the ellipticity of the pump. (d) Measured circular polarization of condensate vs pump ellipticity. Dashed lines mark the region where the condensate initializes stochastically in spin-up or spin-down states in each realization}{figure.3}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces (a) Nonresonant linearly polarized weak probe overlapped with the condensate. (b) Average circular polarization degree vs power of the probe beam. The blue line is a guide to the eye.}}{4}{figure.4}}
\newlabel{fig:ResOnTop}{{4}{4}{(a) Nonresonant linearly polarized weak probe overlapped with the condensate. (b) Average circular polarization degree vs power of the probe beam. The blue line is a guide to the eye}{figure.4}{}}
\newlabel{enum:wl}{{iv}{4}{}{Item.4}{}}
\citation{kavokin_optical_2005,kammann_nonlinear_2012}
\citation{shelykh_semiconductor_2004}
\citation{kammann_nonlinear_2012}
\citation{cristofolini_optical_2013,askitopoulos_robust_2014}
\citation{aleiner_radiative_2012}
\citation{keeling_spontaneous_2008}
\citation{aleiner_radiative_2012}
\newlabel{sec:theory}{{III}{5}{}{section*.5}{}}
\@writefile{toc}{\contentsline {section}{\numberline {III}Spin Bifurcation Theory (Broken Parity)}{5}{section*.5}}
\newlabel{eq:main}{{1}{5}{}{equation.3.1}{}}
\newlabel{eq:maincomp}{{2}{5}{}{equation.3.2alph2}{}}
\newlabel{eq:pseudospinEq}{{3}{5}{}{equation.3.3}{}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {a}Paramagnetic solutions.}{5}{section*.6}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {b}Ferromagnetic solutions.}{5}{section*.7}}
\citation{li_incoherent_2015}
\citation{rayanov_frequency_2015}
\citation{wouters_excitations_2007,keeling_spontaneous_2008,dreismann_coupled_2014}
\citation{wouters_energy_2010}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces  (a) Numerical calculations using Eq.\nobreakspace  {}\ref  {eq:pseudospinEq} for the case when the condensate occupation is below the critical occupation $S_c$ (dotted lines) and when above $S_c$ (solid lines). Blue lines show the occupation of the spin-down component and orange lines show the spin-up component. (b) Numerical calculations of the Stokes parameters at different powers using Eq.\nobreakspace  {}\ref  {eq:pseudospinEq}. (c) Measured power dependence of the condensate Stokes parameters. (d) 2D simulations, with asymmetric initial conditions [$s_z(t=0)<0.01$] show density of the $\psi _\pm $ components of the wave function. Pump spots are marked by dashed lines (see Appendix\nobreakspace  {}\ref  {app:simparam} for parameters). }}{6}{figure.5}}
\newlabel{fig:theoryPD}{{5}{6}{(a) Numerical calculations using Eq.~\ref {eq:pseudospinEq} for the case when the condensate occupation is below the critical occupation $S_c$ (dotted lines) and when above $S_c$ (solid lines). Blue lines show the occupation of the spin-down component and orange lines show the spin-up component. (b) Numerical calculations of the Stokes parameters at different powers using Eq.~\ref {eq:pseudospinEq}. (c) Measured power dependence of the condensate Stokes parameters. (d) 2D simulations, with asymmetric initial conditions [$s_z(t=0)<0.01$] show density of the $\psi _\pm $ components of the wave function. Pump spots are marked by dashed lines (see Appendix~\ref {app:simparam} for parameters)}{figure.5}{}}
\newlabel{eq:Sz_pos}{{5}{6}{}{equation.3.5}{}}
\citation{sadler_spontaneous_2006,stamper-kurn_spinor_2013}
\newlabel{sec:res}{{IV}{7}{}{section*.8}{}}
\@writefile{toc}{\contentsline {section}{\numberline {IV}Resonant excitation}{7}{section*.8}}
\@writefile{toc}{\contentsline {subsection}{\numberline {A}Resonant initialization of spin states}{7}{section*.9}}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces  Measured circular polarization of condensate vs pump ellipticity, for three different gate polarizations. Dashed lines mark the region where the condensate initializes stochastically in spin-up or spin-down states in each realization.  }}{7}{figure.6}}
\newlabel{fig:initialization}{{6}{7}{Measured circular polarization of condensate vs pump ellipticity, for three different gate polarizations. Dashed lines mark the region where the condensate initializes stochastically in spin-up or spin-down states in each realization}{figure.6}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {B}Elliptically-polarized pump: coherent driving}{7}{section*.10}}
\citation{alexeeva_actively_2014}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces  (a) Measured intensity of circular polarization components ($\sigma _\pm $) for adding gate pulse $G$ (intensity shown on above inset). The condensate initializes in the $s_\delimiter "3223379 $ state, due to the asymmetric pumping condition $s_{z,\text  {pump}}=-0.1$. A gate pulse with an opposite circular polarization ($\sigma _+$) is applied. (b) Numerical calculations for (a), showing that during the gate pulse $G=A^2$ the spin-up and spin-down densities oscillate with a $\pi $ phase shift. (c) Time evolution of the pseudospin, showing how the pseudospin orbits around the spin-down stationary state (marked by the blue arrow) when the gate pulse is applied. (d) Same as in (a) but with a fivefold increase in the intensity of the gate. The time-averaged condensate emission is almost circularly unpolarized when the pulse is applied ($\delimiter "426830A s_z \delimiter "526930B =0$). (e) Numerical calculations for (d), showing almost equal amplitude oscillation of the spin-up and spin-down densities. (f) Trajectory of pseudospin, showing that with a strong gate pulse large orbits commence around the two spin-up and spin-down stationary states. (g) Average circular polarization when the gate is on, at different gate intensities. When an opposite polarization gate is applied, $\delimiter "426830A s_z \delimiter "526930B $ converges to zero, whilst it remains unchanged for the same-spin gate. The orange line is a guide to the eye. (h) Numerical calculations of $\delimiter "426830A s_z \delimiter "526930B $ vs normalized pump intensity ($n$ is the condensate occupation). }}{8}{figure.7}}
\newlabel{fig:res}{{7}{8}{(a) Measured intensity of circular polarization components ($\sigma _\pm $) for adding gate pulse $G$ (intensity shown on above inset). The condensate initializes in the $s_\downarrow $ state, due to the asymmetric pumping condition $s_{z,\text {pump}}=-0.1$. A gate pulse with an opposite circular polarization ($\sigma _+$) is applied. (b) Numerical calculations for (a), showing that during the gate pulse $G=A^2$ the spin-up and spin-down densities oscillate with a $\pi $ phase shift. (c) Time evolution of the pseudospin, showing how the pseudospin orbits around the spin-down stationary state (marked by the blue arrow) when the gate pulse is applied. (d) Same as in (a) but with a fivefold increase in the intensity of the gate. The time-averaged condensate emission is almost circularly unpolarized when the pulse is applied ($\langle s_z \rangle =0$). (e) Numerical calculations for (d), showing almost equal amplitude oscillation of the spin-up and spin-down densities. (f) Trajectory of pseudospin, showing that with a strong gate pulse large orbits commence around the two spin-up and spin-down stationary states. (g) Average circular polarization when the gate is on, at different gate intensities. When an opposite polarization gate is applied, $\langle s_z \rangle $ converges to zero, whilst it remains unchanged for the same-spin gate. The orange line is a guide to the eye. (h) Numerical calculations of $\langle s_z \rangle $ vs normalized pump intensity ($n$ is the condensate occupation)}{figure.7}{}}
\newlabel{eq:mainCompRes}{{7}{8}{}{equation.4.7alph2}{}}
\citation{alexeeva_actively_2014}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces  (a) Intensity of the spin-up and -down states as a function of time. Resonant pulse $G$, with opposite circular polarization ($\sigma _+$) switches the circular polarization of the condensate. (b) Despite the slow rise time of our AOM ($\SI {\sim 100}{\nano \second })$, the condensate switches to the opposite spin state in less than $\SI {10}{\nano \second }$ (the limit of our detection), as soon as the intensity crosses the spin-switching threshold. (c) Numerical calculations for (a), showing that the spin switches with a gate pulse with intensity 6 orders of magnitude smaller than that of the condensate. The evolution of the pseudospin is shown in (d). The two attractors, marked by the blue and orange arrows, are the two stationary $s_{\delimiter "3222378 \delimiter "3223379 }$ spin-polarized states. }}{9}{figure.8}}
\newlabel{fig:resSwitch}{{8}{9}{(a) Intensity of the spin-up and -down states as a function of time. Resonant pulse $G$, with opposite circular polarization ($\sigma _+$) switches the circular polarization of the condensate. (b) Despite the slow rise time of our AOM ($\SI {\sim 100}{\nano \second })$, the condensate switches to the opposite spin state in less than $\SI {10}{\nano \second }$ (the limit of our detection), as soon as the intensity crosses the spin-switching threshold. (c) Numerical calculations for (a), showing that the spin switches with a gate pulse with intensity 6 orders of magnitude smaller than that of the condensate. The evolution of the pseudospin is shown in (d). The two attractors, marked by the blue and orange arrows, are the two stationary $s_{\uparrow \downarrow }$ spin-polarized states}{figure.8}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {C}Linearly-polarized pump: spin switching}{9}{section*.11}}
\citation{nozaki_sub-femtojoule_2010}
\citation{paraiso_multistability_2010,cerna_ultrafast_2013}
\citation{wouters_influence_2013}
\citation{paraiso_multistability_2010}
\citation{hill_fast_2004}
\citation{liu_ultra-small_2010}
\newlabel{sec:thermnoise}{{IV\tmspace  +\thinmuskip {.1667em}D}{10}{}{section*.12}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {D}Thermal noise: spin flipping}{10}{section*.12}}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces  (a) Measured spontaneous spin flip rate at different temperatures of the sample. Above the temperature $T_c\simeq \SI {15}{\K }$, the flip rate increases exponentially. The solid line shows the theoretical fit. (b) Calculated dependence of flip rate with normalized noise amplitude. The flip rate increases exponentially as the noise amplitude increases (light region), and eventually becomes linear (dark region). Comparison with (a) shows that the measured flip rates remain below this linear regime. }}{10}{figure.9}}
\newlabel{fig:temp}{{9}{10}{(a) Measured spontaneous spin flip rate at different temperatures of the sample. Above the temperature $T_c\simeq \SI {15}{\K }$, the flip rate increases exponentially. The solid line shows the theoretical fit. (b) Calculated dependence of flip rate with normalized noise amplitude. The flip rate increases exponentially as the noise amplitude increases (light region), and eventually becomes linear (dark region). Comparison with (a) shows that the measured flip rates remain below this linear regime}{figure.9}{}}
\citation{aleiner_radiative_2012}
\citation{read_stochastic_2009}
\citation{lagoudakis_coherent_2010}
\citation{jamet_magnetic_2001,hai_long_2010}
\newlabel{eq:noise}{{8}{11}{}{equation.4.8}{}}
\newlabel{eq:noise2}{{9}{11}{}{equation.4.9}{}}
\newlabel{eq:kramers_rate}{{10}{11}{}{equation.4.10}{}}
\newlabel{sec:conc}{{V}{11}{}{section*.13}{}}
\@writefile{toc}{\contentsline {section}{\numberline {V}Concluding remarks}{11}{section*.13}}
\citation{tsotsis_lasing_2012}
\citation{cristofolini_optical_2013}
\citation{balili_huge_2010,klopotowski_optical_2006}
\citation{aleiner_anisotropic_1992,ivchenko_heavy-light_1996,balili_huge_2010}
\citation{klopotowski_optical_2006}
\@writefile{toc}{\contentsline {section}{\numberline {}Acknowledgments}{12}{section*.14}}
\@writefile{toc}{\appendix }
\newlabel{app:expmethods}{{A}{12}{}{section*.15}{}}
\@writefile{toc}{\contentsline {section}{\numberline {A}Experimental methods}{12}{section*.15}}
\newlabel{app:polsplit}{{B}{12}{}{section*.16}{}}
\@writefile{toc}{\contentsline {section}{\numberline {B}Strain-induced linear polarization splitting}{12}{section*.16}}
\@writefile{lof}{\contentsline {figure}{\numberline {10}{\ignorespaces (a) Energy-resolved emission of the ground state polariton for horizontal (H) and vertical (V) polarizations, split in energy by $\SI {\sim 30}{\ueV }$ (b) Transfer matrix calculations (red) and experimental reflectivity of sample. The lower polariton mode (marked by an arrow), is offset by \SI {10}{\milli \electronvolt } below the center of the stopband. (c) Transfer matrix calculations showing the linewidth difference versus the energy splitting. The linewidth difference is $10\%$ of the energy splitting. }}{13}{figure.10}}
\newlabel{fig:transmat}{{10}{13}{(a) Energy-resolved emission of the ground state polariton for horizontal (H) and vertical (V) polarizations, split in energy by $\SI {\sim 30}{\ueV }$ (b) Transfer matrix calculations (red) and experimental reflectivity of sample. The lower polariton mode (marked by an arrow), is offset by \SI {10}{\milli \electronvolt } below the center of the stopband. (c) Transfer matrix calculations showing the linewidth difference versus the energy splitting. The linewidth difference is $10\%$ of the energy splitting}{figure.10}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {11}{\ignorespaces (a) Absolute degree of polarization vs $\gamma $ for a fixed energy splitting of $\varepsilon =\SI {0.045}{\per \ps }$. (b) Absolute degree of polarization vs energy splitting $\varepsilon $, for the case when $\gamma =0.1 \varepsilon $. }}{13}{figure.11}}
\newlabel{fig:dEgamma}{{11}{13}{(a) Absolute degree of polarization vs $\gamma $ for a fixed energy splitting of $\varepsilon =\SI {0.045}{\per \ps }$. (b) Absolute degree of polarization vs energy splitting $\varepsilon $, for the case when $\gamma =0.1 \varepsilon $}{figure.11}{}}
\newlabel{app:varcross}{{C}{13}{}{section*.17}{}}
\@writefile{toc}{\contentsline {section}{\numberline {C}Variable cross spin saturation}{13}{section*.17}}
\newlabel{Evol2psi2}{{C1}{13}{}{equation.C.1}{}}
\newlabel{EvolPsi}{{C2}{13}{}{equation.C.2}{}}
\newlabel{EvolSpin2}{{C3}{13}{}{equation.C.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1}Linearly polarized condensates (parity conserved)}{13}{section*.18}}
\newlabel{StabEqs}{{C4}{13}{}{equation.C.4}{}}
\newlabel{Lyapun}{{C5}{13}{}{equation.C.5}{}}
\newlabel{W22}{{C6}{13}{}{equation.C.6}{}}
\citation{wouters_spatial_2008,wertz_spontaneous_2010,askitopoulos_polariton_2013}
\@writefile{toc}{\contentsline {subsection}{\numberline {2}Elliptically polarized condensates (parity broken)}{14}{section*.19}}
\newlabel{WLStates2}{{C7}{14}{}{equation.C.7}{}}
\newlabel{EqForS}{{C8}{14}{}{equation.C.8}{}}
\newlabel{sec:particlenumber}{{D}{14}{}{section*.20}{}}
\@writefile{toc}{\contentsline {section}{\numberline {D}Estimate for particle number}{14}{section*.20}}
\newlabel{eq:particlen}{{D1}{14}{}{equation.D.1}{}}
\newlabel{app:reswidth}{{E}{14}{}{section*.21}{}}
\@writefile{toc}{\contentsline {section}{\numberline {E}Resonance width}{14}{section*.21}}
\@writefile{lof}{\contentsline {figure}{\numberline {12}{\ignorespaces  (a) The reduction of the spin-down intensity versus the detuning of the gate laser frequency is shown. A sharp resonance is visible when the laser is in resonance with the condensate. (b) The numerical calculations show a similar resonance effect, with the center of the peak slightly redshifted due to the linear polarization energy splitting $\varepsilon $. }}{14}{figure.12}}
\newlabel{fig:resPeak}{{12}{14}{(a) The reduction of the spin-down intensity versus the detuning of the gate laser frequency is shown. A sharp resonance is visible when the laser is in resonance with the condensate. (b) The numerical calculations show a similar resonance effect, with the center of the peak slightly redshifted due to the linear polarization energy splitting $\ve $}{figure.12}{}}
\citation{zwanzig_nonequilibrium_2001}
\bibdata{mainwholeNotes,main}
\bibcite{deng_condensation_2002}{{1}{2002}{{Deng\ \emph  {et~al.}}}{{Deng, Weihs, Santori, Bloch,\ and\ Yamamoto}}}
\bibcite{kasprzak_bose-einstein_2006}{{2}{2006}{{Kasprzak\ \emph  {et~al.}}}{{Kasprzak, Richard, Kundermann, Baas, Jeambrun, Keeling, Marchetti, Szyma\IeC {\'n}ska, Andr\IeC {\'e}, Staehli, Savona, Littlewood, Deveaud,\ and\ Dang}}}
\bibcite{balili_bose-einstein_2007}{{3}{2007}{{Balili\ \emph  {et~al.}}}{{Balili, Hartwell, Snoke, Pfeiffer,\ and\ West}}}
\bibcite{baumberg_spontaneous_2008}{{4}{2008}{{Baumberg\ \emph  {et~al.}}}{{Baumberg, Kavokin, Christopoulos, Grundy, Butt\IeC {\'e}, Christmann, Solnyshkov, Malpuech, Baldassarri H\IeC {\"o}ger~von H\IeC {\"o}gersthal, Feltin, Carlin,\ and\ Grandjean}}}
\bibcite{ohadi_spontaneous_2012}{{5}{2012}{{Ohadi\ \emph  {et~al.}}}{{Ohadi, Kammann, Liew, Lagoudakis, Kavokin,\ and\ Lagoudakis}}}
\bibcite{nelsen_dissipationless_2013}{{6}{2013}{{Nelsen\ \emph  {et~al.}}}{{Nelsen, Liu, Steger, Snoke, Balili, West,\ and\ Pfeiffer}}}
\newlabel{app:kramers}{{F}{15}{}{section*.22}{}}
\@writefile{toc}{\contentsline {section}{\numberline {F}The Kramers flip rate}{15}{section*.22}}
\newlabel{eq:LEqsS}{{F1}{15}{}{equation.F.1}{}}
\newlabel{NoiseS}{{F2}{15}{}{equation.F.2}{}}
\newlabel{SlowSz}{{F3}{15}{}{equation.F.3}{}}
\newlabel{DeltaU}{{F4}{15}{}{equation.F.4}{}}
\newlabel{KramersR}{{F5}{15}{}{equation.F.5}{}}
\newlabel{app:simparam}{{G}{15}{}{section*.23}{}}
\@writefile{toc}{\contentsline {section}{\numberline {G}Simulations and numerical parameters}{15}{section*.23}}
\@writefile{toc}{\contentsline {section}{\numberline {}References}{15}{section*.24}}
\bibcite{sturm_all-optical_2014}{{7}{2014}{{Sturm\ \emph  {et~al.}}}{{Sturm, Tanese, Nguyen, Flayac, Galopin, Lema\IeC {\^\i }tre, Sagnes, Solnyshkov, Amo, Malpuech,\ and\ Bloch}}}
\bibcite{dreismann_coupled_2014}{{8}{2014}{{Dreismann\ \emph  {et~al.}}}{{Dreismann, Cristofolini, Balili, Christmann, Pinsker, Berloff, Hatzopoulos, Savvidis,\ and\ Baumberg}}}
\bibcite{amo_exciton-polariton_2010}{{9}{2010}{{Amo\ \emph  {et~al.}}}{{Amo, H., AdradosC., HoudreR., GiacobinoE., V.,\ and\ BramatiA.}}}
\bibcite{ballarini_all-optical_2013}{{10}{2013}{{Ballarini\ \emph  {et~al.}}}{{Ballarini, De~Giorgi, Cancellieri, Houdr\IeC {\'e}, Giacobino, Cingolani, Bramati, Gigli,\ and\ Sanvitto}}}
\bibcite{cerna_ultrafast_2013}{{11}{2013}{{Cerna\ \emph  {et~al.}}}{{Cerna, L\IeC {\'e}ger, Para\IeC {\"\i }so, Wouters, Morier-Genoud, Portella-Oberli,\ and\ Deveaud}}}
\bibcite{nguyen_realization_2013}{{12}{2013}{{Nguyen\ \emph  {et~al.}}}{{Nguyen, Vishnevsky, Sturm, Tanese, Solnyshkov, Galopin, Lema\IeC {\^\i }tre, Sagnes, Amo, Malpuech,\ and\ Bloch}}}
\bibcite{bhattacharya_solid_2013}{{13}{2013}{{Bhattacharya\ \emph  {et~al.}}}{{Bhattacharya, Xiao, Das, Bhowmick,\ and\ Heo}}}
\bibcite{schneider_electrically_2013}{{14}{2013}{{Schneider\ \emph  {et~al.}}}{{Schneider, Rahimi-Iman, Kim, Fischer, Savenko, Amthor, Lermer, Wolf, Worschech, Kulakovskii, Shelykh, Kamp, Reitzenstein, Forchel, Yamamoto,\ and\ H\IeC {\"o}fling}}}
\bibcite{buluta_quantum_2009}{{15}{2009}{{Buluta\ and\ Nori}}{{}}}
\bibcite{aleiner_radiative_2012}{{16}{2012}{{Aleiner\ \emph  {et~al.}}}{{Aleiner, Altshuler,\ and\ Rubo}}}
\bibcite{zhang_weak_2015}{{17}{2015}{{Zhang\ \emph  {et~al.}}}{{Zhang, Xie, Wang, Poddubny, Lu, Wang, Gu, Liu, Xu, Shen, Rubo, Altshuler, Kavokin,\ and\ Chen}}}
\bibcite{lagoudakis_stimulated_2002}{{18}{2002}{{Lagoudakis\ \emph  {et~al.}}}{{Lagoudakis, Savvidis, Baumberg, Whittaker, Eastham, Skolnick,\ and\ Roberts}}}
\bibcite{martin_polarization_2002}{{19}{2002}{{Mart\IeC {\'\i }n\ \emph  {et~al.}}}{{Mart\IeC {\'\i }n, Aichmayr, Vi\IeC {\~n}a,\ and\ Andr\IeC {\'e}}}}
\bibcite{kavokin_polarization_2003}{{20}{2003}{{Kavokin\ \emph  {et~al.}}}{{Kavokin, Lagoudakis, Malpuech,\ and\ Baumberg}}}
\bibcite{kavokin_quantum_2004}{{21}{2004}{{Kavokin\ \emph  {et~al.}}}{{Kavokin, Shelykh, Kavokin, Malpuech,\ and\ Bigenwald}}}
\bibcite{renucci_microcavity_2005}{{22}{2005}{{Renucci\ \emph  {et~al.}}}{{Renucci, Amand, Marie, Senellart, Bloch, Sermage,\ and\ Kavokin}}}
\bibcite{krizhanovskii_rotation_2006}{{23}{2006}{{Krizhanovskii\ \emph  {et~al.}}}{{Krizhanovskii, Sanvitto, Shelykh, Glazov, Malpuech, Solnyshkov, Kavokin, Ceccarelli, Skolnick,\ and\ Roberts}}}
\bibcite{gippius_polarization_2007}{{24}{2007}{{Gippius\ \emph  {et~al.}}}{{Gippius, Shelykh, Solnyshkov, Gavrilov, Rubo, Kavokin, Tikhodeev,\ and\ Malpuech}}}
\bibcite{leyder_observation_2007}{{25}{2007}{{Leyder\ \emph  {et~al.}}}{{Leyder, Romanelli, Karr, Giacobino, Liew, Glazov, Kavokin, Malpuech,\ and\ Bramati}}}
\bibcite{paraiso_multistability_2010}{{26}{2010}{{Para\IeC {\"\i }so\ \emph  {et~al.}}}{{Para\IeC {\"\i }so, Wouters, L\IeC {\'e}ger, Morier-Genoud,\ and\ Deveaud-Pl\IeC {\'e}dran}}}
\bibcite{gao_polariton_2012}{{27}{2012}{{Gao\ \emph  {et~al.}}}{{Gao, Eldridge, Liew, Tsintzos, Stavrinidis, Deligeorgis, Hatzopoulos,\ and\ Savvidis}}}
\bibcite{kammann_nonlinear_2012}{{28}{2012}{{Kammann\ \emph  {et~al.}}}{{Kammann, Liew, Ohadi, Cilibrizzi, Tsotsis, Hatzopoulos, Savvidis, Kavokin,\ and\ Lagoudakis}}}
\bibcite{takemura_polaritonic_2014}{{29}{2014{}}{{Takemura\ \emph  {et~al.}}}{{Takemura, Trebaol, Wouters, Portella-Oberli,\ and\ Deveaud}}}
\bibcite{kavokin_microcavities_2007}{{30}{2007}{{Kavokin\ \emph  {et~al.}}}{{Kavokin, Baumberg, Malpuech,\ and\ Laussy}}}
\bibcite{savvidis_angle-resonant_2000}{{31}{2000}{{Savvidis\ \emph  {et~al.}}}{{Savvidis, Baumberg, Stevenson, Skolnick, Whittaker,\ and\ Roberts}}}
\bibcite{wertz_spontaneous_2010}{{32}{2010}{{Wertz\ \emph  {et~al.}}}{{Wertz, Ferrier, Solnyshkov, Johne, Sanvitto, Lema\IeC {\^\i }tre, Sagnes, Grousson, Kavokin, Senellart, Malpuech,\ and\ Bloch}}}
\bibcite{askitopoulos_polariton_2013}{{33}{2013}{{Askitopoulos\ \emph  {et~al.}}}{{Askitopoulos, Ohadi, Kavokin, Hatzopoulos, Savvidis,\ and\ Lagoudakis}}}
\bibcite{bloch_ultracold_2005}{{34}{2005}{{Bloch}}{{}}}
\bibcite{wouters_excitations_2007}{{35}{2007}{{Wouters\ and\ Carusotto}}{{}}}
\bibcite{tosi_sculpting_2012}{{36}{2012}{{Tosi\ \emph  {et~al.}}}{{Tosi, Christmann, Berloff, Tsotsis, Gao, Hatzopoulos, Savvidis,\ and\ Baumberg}}}
\bibcite{shelykh_polarization_2006}{{37}{2006}{{Shelykh\ \emph  {et~al.}}}{{Shelykh, Rubo, Malpuech, Solnyshkov,\ and\ Kavokin}}}
\bibcite{shelykh_semiconductor_2004}{{38}{2004}{{Shelykh\ \emph  {et~al.}}}{{Shelykh, Kavokin, Kavokin, Malpuech, Bigenwald, Deng, Weihs,\ and\ Yamamoto}}}
\bibcite{roumpos_signature_2009}{{39}{2009}{{Roumpos\ \emph  {et~al.}}}{{Roumpos, Lai, Liew, Rubo, Kavokin,\ and\ Yamamoto}}}
\bibcite{li_incoherent_2015}{{40}{}{{Li\ \emph  {et~al.}}}{{Li, Liew, Egorov,\ and\ Ostrovskaya}}}
\bibcite{rubo_suppression_2006}{{41}{2006}{{Rubo\ \emph  {et~al.}}}{{Rubo, Kavokin,\ and\ Shelykh}}}
\bibcite{vladimirova_polariton-polariton_2010}{{42}{2010}{{Vladimirova\ \emph  {et~al.}}}{{Vladimirova, Cronenberger, Scalbert, Kavokin, Miard, Lema\IeC {\^\i }tre, Bloch, Solnyshkov, Malpuech,\ and\ Kavokin}}}
\bibcite{takemura_heterodyne_2014}{{43}{2014{}}{{Takemura\ \emph  {et~al.}}}{{Takemura, Trebaol, Wouters, Portella-Oberli,\ and\ Deveaud}}}
\bibcite{kasprzak_formation_2008}{{44}{2008}{{Kasprzak\ \emph  {et~al.}}}{{Kasprzak, Solnyshkov, Andr\IeC {\'e}, Dang,\ and\ Malpuech}}}
\bibcite{balili_huge_2010}{{45}{2010}{{Balili\ \emph  {et~al.}}}{{Balili, Nelsen, Snoke, Reid, Pfeiffer,\ and\ West}}}
\bibcite{klopotowski_optical_2006}{{46}{2006}{{K\IeC {\l }opotowski\ \emph  {et~al.}}}{{K\IeC {\l }opotowski, Mart\IeC {\'\i }n, Amo, Vi\IeC {\~n}a, Shelykh, Glazov, Malpuech, Kavokin,\ and\ Andr\IeC {\'e}}}}
\bibcite{kavokin_optical_2005}{{47}{2005}{{Kavokin\ \emph  {et~al.}}}{{Kavokin, Malpuech,\ and\ Glazov}}}
\bibcite{cristofolini_optical_2013}{{48}{2013}{{Cristofolini\ \emph  {et~al.}}}{{Cristofolini, Dreismann, Christmann, Franchetti, Berloff, Tsotsis, Hatzopoulos, Savvidis,\ and\ Baumberg}}}
\bibcite{askitopoulos_robust_2014}{{49}{2014}{{Askitopoulos\ \emph  {et~al.}}}{{Askitopoulos, Liew, Ohadi, Hatzopoulos, Savvidis,\ and\ Lagoudakis}}}
\bibcite{keeling_spontaneous_2008}{{50}{2008}{{Keeling\ and\ Berloff}}{{}}}
\bibcite{rayanov_frequency_2015}{{51}{2015}{{Rayanov\ \emph  {et~al.}}}{{Rayanov, Altshuler, Rubo,\ and\ Flach}}}
\bibcite{wouters_energy_2010}{{52}{2010}{{Wouters\ \emph  {et~al.}}}{{Wouters, Liew,\ and\ Savona}}}
\bibcite{sadler_spontaneous_2006}{{53}{2006}{{Sadler\ \emph  {et~al.}}}{{Sadler, Higbie, Leslie, Vengalattore,\ and\ Stamper-Kurn}}}
\bibcite{stamper-kurn_spinor_2013}{{54}{2013}{{Stamper-Kurn\ and\ Ueda}}{{}}}
\bibcite{alexeeva_actively_2014}{{55}{2014}{{Alexeeva\ \emph  {et~al.}}}{{Alexeeva, Barashenkov, Rayanov,\ and\ Flach}}}
\bibcite{nozaki_sub-femtojoule_2010}{{56}{2010}{{Nozaki\ \emph  {et~al.}}}{{Nozaki, Tanabe, Shinya, Matsuo, Sato, Taniyama,\ and\ Notomi}}}
\bibcite{wouters_influence_2013}{{57}{2013}{{Wouters\ \emph  {et~al.}}}{{Wouters, Para\IeC {\"\i }so, L\IeC {\'e}ger, Cerna, Morier-Genoud, Portella-Oberli,\ and\ Deveaud-Pl\IeC {\'e}dran}}}
\bibcite{hill_fast_2004}{{58}{2004}{{Hill\ \emph  {et~al.}}}{{Hill, Dorren, de~Vries, Leijtens, den Besten, Smalbrugge, Oei, Binsma, Khoe,\ and\ Smit}}}
\bibcite{liu_ultra-small_2010}{{59}{2010}{{Liu\ \emph  {et~al.}}}{{Liu, Kumar, Huybrechts, Spuesens, Roelkens, Geluk, de~Vries, Regreny, Van~Thourhout, Baets,\ and\ Morthier}}}
\bibcite{read_stochastic_2009}{{60}{2009}{{Read\ \emph  {et~al.}}}{{Read, Liew, Rubo,\ and\ Kavokin}}}
\bibcite{lagoudakis_coherent_2010}{{61}{2010}{{Lagoudakis\ \emph  {et~al.}}}{{Lagoudakis, Pietka, Wouters, Andr\IeC {\'e},\ and\ Deveaud-Pl\IeC {\'e}dran}}}
\bibcite{jamet_magnetic_2001}{{62}{2001}{{Jamet\ \emph  {et~al.}}}{{Jamet, Wernsdorfer, Thirion, Mailly, Dupuis, M\IeC {\'e}linon,\ and\ P\IeC {\'e}rez}}}
\bibcite{hai_long_2010}{{63}{2010}{{Hai\ \emph  {et~al.}}}{{Hai, Ohya,\ and\ Tanaka}}}
\bibcite{tsotsis_lasing_2012}{{64}{2012}{{Tsotsis\ \emph  {et~al.}}}{{Tsotsis, Eldridge, Gao, Tsintzos, Hatzopoulos,\ and\ Savvidis}}}
\bibcite{aleiner_anisotropic_1992}{{65}{1992}{{Aleiner\ and\ Ivchenko}}{{}}}
\bibcite{ivchenko_heavy-light_1996}{{66}{1996}{{Ivchenko\ \emph  {et~al.}}}{{Ivchenko, Kaminski,\ and\ R\IeC {\"o}ssler}}}
\bibcite{wouters_spatial_2008}{{67}{2008}{{Wouters\ \emph  {et~al.}}}{{Wouters, Carusotto,\ and\ Ciuti}}}
\bibcite{zwanzig_nonequilibrium_2001}{{68}{2001}{{Zwanzig}}{{}}}
\bibstyle{apsrev4-1}
\citation{REVTEX41Control}
\citation{apsrev41Control}
\newlabel{LastBibItem}{{68}{18}{}{section*.24}{}}
\newlabel{LastPage}{{}{18}{}{}{}}

